Fast optical flares from M dwarfs detected by a one-second-cadence survey with Tomo-e Gozen

We report a one-second-cadence wide-field survey for M-dwarf flares using the Tomo-e Gozen camera mounted on the Kiso Schmidt telescope. We detect 22 flares from M3-M5 dwarfs with rise times and amplitudes ranging from $5\, \mathrm{sec} \lesssim t_\mathrm{rise} \lesssim 100\,\mathrm{sec}$ and $0.5 \lesssim \Delta F/F_{\star} \lesssim 20$, respectively. The flare light curves mostly show steeper rises and shallower decays than those obtained from the Kepler one-minute cadence data and tend to have flat peak structures. Assuming a blackbody spectrum with temperatures of $9,000-15,000\,\mathrm{K}$, the peak luminosities and bolometric energies are estimated to be $10^{29}\,\mathrm{erg\,sec^{-1}} \lesssim L_\mathrm{peak} \lesssim 10^{31}\,\mathrm{erg\,sec^{-1}}$ and $10^{31}\,\mathrm{erg} \lesssim E_{\rm bol} \lesssim 10^{34}\,\mathrm{erg}$, which constitutes the bright end of fast optical flares for M dwarfs. We confirm that more than 90\% of the host stars of the detected flares are magnetically active based on their H$\alpha$ emission line intensities obtained by LAMOST. The estimated occurrence rate of the detected flares is $\sim 0.7$ per day per an active star, indicating they are common in magnetically active M dwarfs. We argue that the flare light curves can be explained by the chromospheric compression model; the rise time is broadly consistent with the Alfv\'en transit time of a magnetic loop with a length scale of $l_\mathrm{loop} \sim 10^4\,\mathrm{km}$ and a field strength of $1,000\,\mathrm{G}$, while the decay time is likely determined by the radiative cooling of the compressed chromosphere down to near the photosphere with a temperature of $\gtrsim 10,000\,\mathrm{K}$. These flares from M dwarfs could be a major contamination source for a future search of fast optical transients of unknown types.

==> table_flare_mcmc_paras.tex <==
\begin{splitdeluxetable}{c|cccccBcccccc} 
\caption{Flare parameters } \label{table:flare_paras} 
 \setlength{\tabcolsep}{5pt} 
 \tabletypesize{\scriptsize} \tablehead{ 
\colhead{TIC ID} & \colhead{$f_{\rm peak}$}& \colhead{$t_{\rm rise}$ [sec]}& \colhead{$t_{\rm peak, const}$ [sec]}& \colhead{$t_{\rm FWHM}$ [sec]}& \colhead{$\tau_{\rm fast}$ [sec]}& \colhead{$\tau_{\rm slow}$ [sec]}& \colhead{$F_{\rm fast}$}& \colhead{$L_{\rm max}$[erg/s]}& \colhead{$l_{\rm max}$[km]}& \colhead{$E_{\rm bol}$[erg]}& \colhead{$E_{\rm tomoe}$[erg]}} \startdata 
15904458 (1st peak)& $0.47 \pm ^{0.03}_{-0.04}$& $36.90 \pm ^{1.99}_{-1.93}$& $3.16 \pm ^{2.90}_{-2.09}$& $38.63 \pm ^{6.04}_{-6.14}$& $32.78 \pm ^{3.21}_{-2.92}$& $711.43 \pm ^{34.42}_{-31.98}$& $0.75 \pm ^{0.08}_{-0.06}$& $2.5 \times 10^{30}$& $2.5 \times 10^{4}$& $5.6 \times 10^{32}$& $2.0 \times 10^{32}$ \\ 
15904458 (2nd peak)& $0.94 \pm ^{0.04}_{-0.03}$& $29.13 \pm ^{1.81}_{-2.03}$& $2.12 \pm ^{1.44}_{-1.51}$& $14.95 \pm ^{1.28}_{-1.41}$& $13.62 \pm ^{1.39}_{-1.94}$& $711.43 \pm ^{34.42}_{-31.98}$& $0.85 \pm ^{0.04}_{-0.06}$& $5.0 \times 10^{30}$& $3.6 \times 10^{4}$& $6.8 \times 10^{32}$& $2.4 \times 10^{32}$ \\ 
17198188& $0.39 \pm ^{0.05}_{-0.04}$& $13.76 \pm ^{5.87}_{-7.62}$& $3.68 \pm ^{4.29}_{-2.60}$& $38.32 \pm ^{8.28}_{-7.12}$& $38.86 \pm ^{8.41}_{-7.27}$& $2241.52 \pm ^{1226.16}_{-1122.58}$& $0.87 \pm ^{0.02}_{-0.03}$& $1.5 \times 10^{29}$& $6.1 \times 10^{3}$& $4.9 \times 10^{31}$& $1.7 \times 10^{31}$ \\ 
18376490& $0.25 \pm ^{0.02}_{-0.02}$& $39.07 \pm ^{6.76}_{-7.06}$& $4.54 \pm ^{4.51}_{-3.22}$& $39.85 \pm ^{10.99}_{-9.47}$& $23.88 \pm ^{8.67}_{-7.39}$& $827.20 \pm ^{362.46}_{-178.97}$& $0.64 \pm ^{0.04}_{-0.05}$& $3.9 \times 10^{29}$& $9.9 \times 10^{3}$& $1.3 \times 10^{32}$& $4.6 \times 10^{31}$ \\ 
20536892 (1st peak)& $2.91 \pm ^{0.04}_{-0.04}$& $37.63 \pm ^{2.15}_{-2.40}$& $1.53 \pm ^{1.59}_{-1.08}$& $83.63 \pm ^{2.65}_{-2.60}$& $88.70 \pm ^{7.25}_{-7.58}$& $415.27 \pm ^{124.60}_{-72.36}$& $0.76 \pm ^{0.06}_{-0.06}$& $1.9 \times 10^{31}$& $6.9 \times 10^{4}$& $3.4 \times 10^{33}$& $1.2 \times 10^{33}$ \\ 
21286088& \nodata& $37.53 \pm ^{1.15}_{-1.40}$& $1.69 \pm ^{2.56}_{-1.07}$& $96.84 \pm ^{2.66}_{-2.16}$& $118.51 \pm ^{2.16}_{-2.28}$& $1150.34 \pm ^{42.25}_{-52.45}$& $0.90 \pm ^{0.00}_{-0.00}$& $3.4 \times 10^{31}$& $9.4 \times 10^{4}$& $8.4 \times 10^{33}$& $3.0 \times 10^{33}$ \\ 
21286574& $0.32 \pm ^{0.00}_{-0.00}$& $9.42 \pm ^{8.87}_{-4.19}$& $19.02 \pm ^{9.00}_{-6.91}$& $52.48 \pm ^{8.95}_{-6.97}$& $30.93 \pm ^{1.60}_{-1.39}$& $298.28 \pm ^{16.23}_{-13.36}$& $0.72 \pm ^{0.01}_{-0.01}$& $2.9 \times 10^{30}$& $2.7 \times 10^{4}$& $3.2 \times 10^{32}$& $1.1 \times 10^{32}$ \\ 
46305452& $0.14 \pm ^{0.01}_{-0.01}$& $74.94 \pm ^{31.50}_{-24.52}$& $62.63 \pm ^{24.48}_{-35.50}$& $121.57 \pm ^{16.90}_{-21.10}$& $67.73 \pm ^{25.23}_{-24.54}$& $1824.12 \pm ^{3196.79}_{-1591.63}$& $0.85 \pm ^{0.04}_{-0.17}$& $9.4 \times 10^{29}$& $1.5 \times 10^{4}$& $3.4 \times 10^{32}$& $1.2 \times 10^{32}$ \\ 
55288759& $0.05 \pm ^{0.01}_{-0.01}$& $6.11 \pm ^{2.40}_{-1.49}$& $2.14 \pm ^{2.10}_{-1.47}$& $20.36 \pm ^{4.33}_{-4.18}$& $20.91 \pm ^{4.31}_{-5.06}$& $773.47 \pm ^{894.84}_{-492.11}$& $0.88 \pm ^{0.01}_{-0.04}$& $3.8 \times 10^{29}$& $9.9 \times 10^{3}$& $4.4 \times 10^{31}$& $1.6 \times 10^{31}$ \\ 
98751507& $0.15 \pm ^{0.01}_{-0.01}$& $5.96 \pm ^{4.52}_{-1.55}$& $11.70 \pm ^{2.88}_{-3.83}$& $22.31 \pm ^{3.66}_{-3.86}$& $8.08 \pm ^{5.45}_{-2.29}$& $45.52 \pm ^{21.24}_{-13.93}$& $0.64 \pm ^{0.15}_{-0.19}$& $4.5 \times 10^{29}$& $1.1 \times 10^{4}$& $1.1 \times 10^{31}$& $4.0 \times 10^{30}$ \\ 
119031076& $0.11 \pm ^{0.01}_{-0.00}$& $8.84 \pm ^{2.90}_{-2.21}$& $6.37 \pm ^{1.67}_{-1.92}$& $20.88 \pm ^{1.83}_{-1.77}$& $13.60 \pm ^{2.38}_{-2.12}$& $154.38 \pm ^{25.70}_{-20.43}$& $0.75 \pm ^{0.04}_{-0.04}$& $3.8 \times 10^{29}$& $9.9 \times 10^{3}$& $2.1 \times 10^{31}$& $7.4 \times 10^{30}$ \\ 
121638493& $0.34 \pm ^{0.11}_{-0.13}$& $17.02 \pm ^{10.39}_{-8.50}$& $5.92 \pm ^{56.30}_{-4.24}$& $35.77 \pm ^{47.11}_{-21.01}$& $9.02 \pm ^{33.18}_{-4.95}$& $94.64 \pm ^{298.69}_{-24.97}$& $0.55 \pm ^{0.31}_{-0.22}$& $1.6 \times 10^{30}$& $2.0 \times 10^{4}$& $9.2 \times 10^{31}$& $3.3 \times 10^{31}$ \\ 
185243119& $3.32 \pm ^{0.07}_{-0.07}$& $99.73 \pm ^{8.90}_{-7.28}$& $14.82 \pm ^{7.43}_{-7.86}$& $205.25 \pm ^{7.07}_{-7.57}$& $260.61 \pm ^{10.43}_{-18.63}$& $290.32 \pm ^{33.33}_{-12.20}$& $0.55 \pm ^{0.26}_{-0.32}$& $1.7 \times 10^{31}$& $6.6 \times 10^{4}$& $5.5 \times 10^{33}$& $2.0 \times 10^{33}$ \\ 
203228080& $0.33 \pm ^{0.04}_{-0.03}$& $34.54 \pm ^{12.08}_{-11.69}$& $24.58 \pm ^{24.68}_{-16.93}$& $137.52 \pm ^{26.40}_{-27.36}$& $121.81 \pm ^{27.17}_{-38.58}$& $1443.87 \pm ^{6654.13}_{-1181.92}$& $0.84 \pm ^{0.05}_{-0.37}$& $1.9 \times 10^{30}$& $2.2 \times 10^{4}$& $6.5 \times 10^{32}$& $2.3 \times 10^{32}$ \\ 
243017627& $0.12 \pm ^{0.01}_{-0.01}$& $29.74 \pm ^{10.39}_{-8.44}$& $90.65 \pm ^{6.33}_{-11.05}$& $190.94 \pm ^{14.90}_{-16.15}$& $90.46 \pm ^{47.89}_{-60.15}$& $230.35 \pm ^{100.90}_{-41.92}$& $0.42 \pm ^{0.34}_{-0.21}$& $6.6 \times 10^{29}$& $1.3 \times 10^{4}$& $1.2 \times 10^{32}$& $4.4 \times 10^{31}$ \\ 
251725681& $0.04 \pm ^{0.01}_{-0.01}$& $11.73 \pm ^{18.37}_{-6.42}$& $16.33 \pm ^{11.06}_{-11.46}$& $75.05 \pm ^{56.75}_{-28.07}$& $26.82 \pm ^{44.00}_{-17.01}$& $938.83 \pm ^{2830.20}_{-417.65}$& $0.58 \pm ^{0.11}_{-0.12}$& $3.3 \times 10^{29}$& $9.3 \times 10^{3}$& $1.4 \times 10^{32}$& $4.9 \times 10^{31}$ \\ 
315617164& $0.22 \pm ^{0.05}_{-0.04}$& $8.67 \pm ^{6.53}_{-3.64}$& $18.58 \pm ^{14.29}_{-13.92}$& $36.88 \pm ^{10.49}_{-12.18}$& $14.97 \pm ^{12.47}_{-8.55}$& $54.43 \pm ^{88.75}_{-23.44}$& $0.66 \pm ^{0.20}_{-0.36}$& $9.5 \times 10^{29}$& $1.6 \times 10^{4}$& $3.1 \times 10^{31}$& $1.1 \times 10^{31}$ \\ 
358561826& $1.16 \pm ^{0.06}_{-0.06}$& $56.28 \pm ^{5.76}_{-5.76}$& $6.37 \pm ^{4.18}_{-3.63}$& $27.68 \pm ^{5.30}_{-4.62}$& $13.29 \pm ^{2.02}_{-2.04}$& $553.31 \pm ^{80.06}_{-62.60}$& $0.62 \pm ^{0.03}_{-0.03}$& $2.4 \times 10^{30}$& $2.5 \times 10^{4}$& $6.0 \times 10^{32}$& $2.1 \times 10^{32}$ \\ 
358573853& $0.11 \pm ^{0.03}_{-0.03}$& $29.64 \pm ^{46.65}_{-10.45}$& $8.26 \pm ^{69.59}_{-5.71}$& $88.56 \pm ^{31.83}_{-48.33}$& $8.59 \pm ^{81.11}_{-3.82}$& $225.68 \pm ^{356.82}_{-39.99}$& $0.44 \pm ^{0.33}_{-0.13}$& $2.9 \times 10^{29}$& $8.6 \times 10^{3}$& $4.2 \times 10^{31}$& $1.5 \times 10^{31}$ \\ 
366485128& $0.21 \pm ^{0.02}_{-0.02}$& $83.31 \pm ^{25.70}_{-44.75}$& $34.57 \pm ^{33.64}_{-24.27}$& $285.22 \pm ^{84.25}_{-80.87}$& $183.48 \pm ^{123.53}_{-139.70}$& $4993.99 \pm ^{12299.37}_{-4209.18}$& $0.67 \pm ^{0.12}_{-0.28}$& $1.7 \times 10^{30}$& $2.1 \times 10^{4}$& $3.0 \times 10^{33}$& $1.1 \times 10^{33}$ \\ 
374272810& $0.17 \pm ^{0.01}_{-0.01}$& $33.77 \pm ^{7.30}_{-11.18}$& $51.56 \pm ^{9.00}_{-11.68}$& $160.88 \pm ^{23.80}_{-21.42}$& $45.73 \pm ^{42.25}_{-22.13}$& $844.25 \pm ^{758.99}_{-178.52}$& $0.50 \pm ^{0.12}_{-0.07}$& $2.6 \times 10^{29}$& $8.1 \times 10^{3}$& $1.2 \times 10^{32}$& $4.3 \times 10^{31}$ \\ 
380197137& $1.10 \pm ^{0.07}_{-0.06}$& $10.50 \pm ^{2.52}_{-1.88}$& $4.97 \pm ^{1.08}_{-1.41}$& $9.75 \pm ^{1.21}_{-1.43}$& $4.06 \pm ^{1.03}_{-0.89}$& $73.58 \pm ^{16.48}_{-12.54}$& $0.77 \pm ^{0.04}_{-0.04}$& $1.5 \times 10^{30}$& $2.0 \times 10^{4}$& $3.8 \times 10^{31}$& $1.4 \times 10^{31}$ \\ 
435904068& $0.18 \pm ^{0.03}_{-0.02}$& $33.26 \pm ^{10.54}_{-12.86}$& $5.27 \pm ^{6.48}_{-3.75}$& $31.08 \pm ^{10.38}_{-9.45}$& $26.30 \pm ^{10.18}_{-18.60}$& $164.21 \pm ^{458.27}_{-96.96}$& $0.79 \pm ^{0.09}_{-0.36}$& $1.4 \times 10^{30}$& $1.9 \times 10^{4}$& $9.7 \times 10^{31}$& $3.5 \times 10^{31}$ \\ 
 \enddata 
\end{splitdeluxetable} 

